Beyond VQA: Generating Multi-word Answer and Rationale to Visual Questions

Visual Question Answering is a multi-modal task that aims to measure high-level visual understanding. Contemporary VQA models are restrictive in the sense that answers are obtained via classification over a limited vocabulary (in the case of open-ended VQA), or via classification over a set of multiple-choice-type answers. In this work, we present a completely generative formulation where a multi-word answer is generated for a visual query. To take this a step forward, we introduce a new task: ViQAR (Visual Question Answering and Reasoning), wherein a model must generate the complete answer and a rationale that seeks to justify the generated answer. We propose an end-to-end architecture to solve this task and describe how to evaluate it. We show that our model generates strong answers and rationales through qualitative and quantitative evaluation, as well as through a human Turing Test.

==> CVPR/sections/introduction_copy.tex <==
%\vspace{-18pt}
\section{Introduction}
\label{sec:intro}
%\vspace{-7pt}

Visual Question Answering(VQA)~\cite{VQA} is a vision-language task that has seen a lot of attention in recent years. In general, the VQA task consists of either open-ended or multiple choice answers to a question about the image.
There are an increasing number of models devoted to obtaining the best possible performance on benchmark VQA datasets, which intend to measure visual understanding based on visual questions. Most existing works perform VQA by using an attention mechanism and combining features from two modalities for predicting answers. However, answers in existing VQA datasets and models are largely one-word answers (average length is 1.1 words), which gives existing models the freedom to treat answer generation as a classification task. For the open-ended VQA task, the top-K answers are chosen, and models perform classification over this vocabulary. 
 
However, many questions which require commonsense reasoning cannot be answered in a single word. A textual answer for a sufficiently complicated question may need to be a sentence. For example, a question of the type "What will happen...." usually cannot be answered completely using a single word. Fig \ref{fig:VCR_generative} shows examples of such questions where multi-word answers are required (the answers and rationales in this figure are generated by our model in this work). Current VQA systems are not well-suited for questions of this type. To reduce this gap, more recently, the Visual Commonsense Reasoning (VCR) task~\cite{Zellers2018FromRT,Lu2019ViLBERTPT,Dua2019DROPAR,Zheng2019ReasoningVD,Talmor2018CommonsenseQAAQ} was proposed, which requires a greater level of visual understanding and an
% \begin{figure*}
% \centering
% %\vspace{-6pt}
% % %\vspace{-17pt}
% \includegraphics[width =0.95\textwidth,height=0.22\textwidth ]{figures/many_ans_5739_new.pdf}
% %\vspace{-4pt}
% \caption{An example from the VCR dataset \cite{Zellers2018FromRT} shows that there can be many correct multi-word answers to a question, which makes classification setting restrictive. The highlighted option is the correct option present in the VCR dataset, the rest are examples of plausible correct answers.}
% % %\vspace{-17pt}
% %\vspace{-10pt}
% \label{fig:VCR_example_manychoices}
% \end{figure*}
\begin{figure*}
\centering
\subfloat[\label{fig:VCR_example_manychoices}]{\includegraphics[width =0.92\textwidth ]{figures/many_ans_5739_new.pdf}}
\vfill
\vspace{-6pt}
\subfloat[\label{fig:VCR_generative}]{\includegraphics[width =0.95\textwidth]{figures/ijcai.pdf}}
\vspace{-6pt}
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.4cm]{journal/appendix/figures_appendix/failure_cases/Supp_failure7_15521_.pdf}\label{fig:q1}} \hfill
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.4cm]{journal/appendix/figures_appendix/failure_cases/Supp_failure4_9778_.pdf}\label{fig:q2}} 
\caption{(a) An example from the VCR dataset \cite{Zellers2018FromRT} shows that there can be many correct multi-word answers to a question, which makes classification setting restrictive. The highlighted option is the correct option present in the VCR dataset, the rest are examples of plausible correct answers. (b) Given an image and a question about the image, we \textbf{generate} a natural language answer and reason that explains why the answer was generated. The images shown above are examples of outputs that our proposed model generates. These examples also illustrate the kind of visual questions for which a single-word answer is insufficient. Contemporary VQA models handle even such kinds of questions only in a classification setting, which is limiting.}
%\vspace{-11pt}
\end{figure*}
ability to reason about the world. More interestingly, the VCR dataset features multi-word answers, with an average answer length of $7.55$ words. However, VCR is still a classification task, where the correct answer is chosen from a set of four answers. Models which solve classification tasks simply need to pick an answer in the case of VQA, or an answer and a rationale for VCR. However, when multi-word answers are required for a visual question, options are not sufficient, since the same 'correct' answer can be paraphrased in a multitude of ways, each having the same semantic meaning but differing in grammar. Fig \ref{fig:VCR_example_manychoices} shows an image from the VCR dataset, where the first highlighted answer is the correct one among a set of four options provided in the dataset. The remaining three answers in the figure are included by us here (not in the dataset) as other plausible correct answers. Existing VQA models are fundamentally limited by picking a right option, rather to answer in a more natural manner. % Besides, classification models for multi-word answers may be prone to memorization or lack high-level reasoning.  
% \begin{figure*}
% \centering
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.2cm]{figures/vcr_many_ans(5739).pdf}\label{fig:q1}}\hfill
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.2cm]{figures/vcr_many_ans(3440).pdf}\label{fig:q1}}\\
% %\vspace{-9pt}
% \caption{Examples from the VCR dataset to demonstrate that there can be many more correct answers for a question, which makes the classification setting very restrictive.}
% \label{fig:VCR_example_manychoices}
% \end{figure*}
Moreover, since the number of possible `correct' options in multi-word answer settings can be large (as evidenced by Fig \ref{fig:VCR_example_manychoices}), we propose that for richer answers, one would need to move away from the traditional classification setting, and instead let our model \textit{generate the answer} to a given question. We hence propose a new task which takes a generative approach to multi-word VQA in this work. 

Humans when answering questions often use a rationale to justify the answer. In certain cases, humans answer directly from memory (perhaps through associations) and then provide a post-hoc rationale, which could help improve the answer too - thus suggesting an interplay between an answer and its rationale. Following this cue, we also propose to generate a rationale along with the answer which serves two purposes: (i) it helps justify the generated answer to end-users; and (ii) it helps generate a better answer.
Going beyond contemporary efforts in VQA, we hence propose, for the first time to the best of our knowledge, an approach that automatically generates both multi-word answers and an accompanying rationale, that also serves as a textual justification for the answer. We term this task  \pnamefull ( \pname) and propose an end-to-end methodology to address this task.  This task is especially important in critical AI tasks such as VQA in the medical domain, where simply answering questions about the medical images is not sufficient. Instead, generating a rationale to justify the generated answer will help patients/doctors trust the models outcome and also understand the exact cause for the disease.

% This task is especially important in critical AI tasks such as  VQA in the medical domain. Answering questions about medical images is not sufficient. Instead,  a rationale along with the answer will provide justification to the patients/doctors and thus help them understand the exact cause for the disease and may also help the end user trust the model.}

% \begin{figure*}
% \centering
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.2cm]{figures/vcr_many_ans(5739).pdf}\label{fig:q1}}\hfill
% \subfloat{\includegraphics[width=0.49\linewidth,height=2.2cm]{figures/vcr_many_ans(3440).pdf}\label{fig:q1}}\\
% %\vspace{-9pt}
% \caption{Examples from the VCR dataset to demonstrate that there can be many more correct answers for a question, which makes the classification setting very restrictive.}
% \label{fig:VCR_example_manychoices}
% \end{figure*}
% \begin{figure*}
% %\vspace{-2pt}
% \centering
% \includegraphics[width =0.95\textwidth]{figures/ijcai.pdf}
% \vspace{-4pt}
% \caption{Given an image and a question about the image, we \textbf{generate} a natural language answer and reason that explains why the answer was generated. The images shown above are examples of outputs that our proposed model generates. 
% %To the best of our knowledge, this is the first such effort of automatically generating a multi-word answer and rationale to a visual question, instead of picking answers from a pre-defined list.
% These examples also illustrate the kind of visual questions for which a single-word answer is insufficient. Contemporary VQA models handle even such kinds of questions only in a classification setting, which is limiting.}
% %\vspace{-8pt}
% \label{fig:VCR_generative}
% \end{figure*}
In addition to formalizing this new task, we provide a simple yet reasonably effective model consisting of four sequentially arranged recurrent networks to address this challenge. The model can be seen as having two parts: a generation module (GM), which comprises of the first two sequential recurrent networks, and a refinement module (RM), which comprises of the final two sequential recurrent networks. The GM first generates an answer, using which it generates a rationale that explains the answer. The RM generates a \textit{refined} answer based on the rationale generated by GM. The refined answer is further used to generate a refined rationale. Our overall model design is motivated by the way humans think about answers to questions, wherein the answer and rationale are often mutually dependent on each other (one could motivate the other and also refine the other). We seek to model this dependency by first generating an answer-rationale pair and then using them as priors to regenerate a refined answer and rationale. We train our model on the VCR dataset, which contains open-ended visual questions along with answers and rationales. Considering this is a generative task, we evaluate our methodology by comparing our generated answer/rationale with the ground truth answer/rationale on correctness and goodness of the generated content using generative language metrics, as well as by human Turing Tests. %Considering the difficulty of this task, we observe promising qualitative and quantitative results, as presented later in this paper.

%\vspace{-1mm}
Our main contributions in this work can be summarized as follows: (i) We propose a new task \pname\ that seeks to open up a new dimension of Visual Question Answering tasks, by moving to a completely generative paradigm; (ii) We propose a simple and effective model based on generation and iterative refinement for \pname (which could serve as a baseline to the community); (iii) Considering generative models in general can be difficult to evaluate, we provide a discussion on how to evaluate such models, as well as study a comprehensive list of evaluation metrics for this task; (iv) We conduct a suite of experiments which show promise of the proposed model for this task, and also perform ablation studies of various choices and components to study the effectiveness of the proposed methodology on \pname. %\redc{In summary the main focus of this work is to propose a new generative task that goes beyond traditional VQA, solve it with a simple yet effective baseline model, and provide a baseline for further efforts.} 
We believe that this work could lead to further efforts on common-sense answer and rationale generation in vision tasks in the near future. To the best of our knowledge, this is the first such effort of automatically generating a multi-word answer and rationale to a visual question, instead of picking answers from a pre-defined list.
% %Deep learning models are a quintessential example of black-box methods where it is very hard to see why the model generates the output it does. Over recent years, there has been a rise in the need for explainable deep learning models that have led to several efforts in justification and introspective explanation systems~\cite{Guan2019TowardsAD,Liu2018TowardsEN,Gilpin2018ExplainingEA,Chen2018ExplainingNN,Yosinski2015UnderstandingNN,Hendricks2016GeneratingVE,Doersch2015WhatMP,Berg2013HowDY,Escorcia2015OnTR,Zeiler2013VisualizingAU,Ghosh2019GeneratingNL,Hendricks2018GroundingVE}. Introspective explanations can provide insight into a model’s decision process, though it may be harder for a human unfamiliar with deep learning to understand. 
% %Therefore, end-users always prefer deep learning models with a human-understandable justification of the decision. Despite several efforts towards explanation systems, the need to generate a human-understandable rationale for the generation of long answers from a neural network model has remained.%
% In this work, we propose a new task and methodology for automatically generating a multi-word answer and rationale for a visual question, thus going beyond traditional Visual Question Answering~\cite{Antol2015VQAVQ}.}
% %  Justification systems can potentially be clearer to end-users who are not familiar with deep models. model may not directly reflect the model’s decision
% % process, it can provide straightforward explanations which
% % are easy to understand by end-users
% \bluec{Visual Question Answering (VQA)~\cite{Thomason2018ShiftingTB,Lu2019ViLBERTPT,Storks2019CommonsenseRF,Jang2017TGIFQATS,Lei2018TVQALC} is a vision-language task that has seen a lot of attention in recent years. There are an increasing number of models devoted to obtaining the best possible performance on benchmark VQA datasets, which intend to measure visual understanding based on visual questions. Most existing works perform VQA by using attention
% mechanism and combining features from two modalities for predicting answers. 
% % Also more recently VQA-E\cite{Li2018VQAEEE} and multimodal explanation\cite{Papineni2001BleuAM}   has been proposed to generate an explanation with the predicted answer.
% Although promising performance has been reported, there is still a huge gap for humans to understand the models decision without any explanation. 
% % Also,
% To reduce this gap, more recently, the Visual Commonsense Reasoning (VCR) task~\cite{Zellers2018FromRT,Lu2019ViLBERTPT,Dua2019DROPAR,Zheng2019ReasoningVD,Talmor2018CommonsenseQAAQ,Lin2019KagNetKG} has been proposed, which requires a greater level of visual understanding and an ability to reason about the world. However, both VQA and VCR are posed as multiple-choice questions, which in effect, reduces them to classification problems, i.e., models which solve these tasks simply need to pick an answer in the case of VQA, or an answer and a rationale for VCR. Such models may be prone to memorization or lack high-level visual reasoning itself. Even more recent efforts such as VQA-E~\cite{Li2018VQAEEE} and Multi-modal explanations\cite{Papineni2001BleuAM,Patro2020RobustEF} have been undertaken towards making such models less obscure by making the model generate a justification for its predicted answer.
% % , and by \cite{Selvaraju2020SQuINTingAV} via linking Reasoning questions with sets of appropriate Perception sub-questions encouraging  image  regions  important for the sub-question to play a role in answering the main Reasoning question.
% However, the answers in these are open-ended(generally yes/no, numerical, single-word answers), and the problem persists since all the questions cannot be answered with one word and existing work (VQA-E and Multi-modal explanation) fails to provide  multi-word answers.  VCR has a longer answer, but they are in the form of options and are restrictive as there can be many such correct multi-word answers. 
% % This leads us to generate natural-language answers and rationale to a question.
% To go beyond the contemporary efforts, we propose, for the first time to the best of our knowledge, a task that requires the automatic generation of both multi-word answers and an accompanying rationale that seeks to justify the said answer for a given visual query. It will lead to more interpretable VQA models. We term this task \pnamefull(\pname). We also propose an end-to-end methodology to address this task.}
% 
% Our model to address this task consists of four sequentially arranged recurrent networks. The model can be seen as having two parts: a generation module (GM), which comprises of the first two sequential recurrent networks, and a refinement module (RM), which comprises of the final two sequential recurrent networks. The GM first generates an answer, using which it generates a rationale that explains the answer. The RM generates a \textit{refined} answer based on the rationale generated by GM. The refined answer is further used to generate a refined rationale. Our model is motivated by the way humans think about answers to questions, wherein the answer and rationale are often mutually dependent on each other. We seek to model this cyclic dependency by first generating the answer-rationale pair, and then using them as priors to regenerate a refined answer and rationale. We train our model on the VCR dataset, which contains open-ended visual questions along with answers and rationales. Considering this is a generative task, we evaluate our methodology by comparing our generated
% answer/rationale with the ground truth answer/rationale on correctness and goodness of the generated content, as well as by human Turing Tests. Considering the difficulty of this task, we observe promising qualitative and quantitative results, as presented later in this paper.
% 
% Our main contributions in this work are three-fold: (i) Firstly, we propose a new task \pname  that aims to provide a new direction to interpretable models that can perform visual reasoning and provide human-understandable rationale; (ii) Secondly, we propose an end-to-end methodology for \pname, obtain promising results, and perform ablation studies on our methodology to study its effectiveness on \pname; and (iii) We discuss how to evaluate such models, and provide performance metrics for this task. We believe that this work could lead to further efforts on human-understandable answer and rationale generation in vision tasks in the near future.
% 
%%\vspace{-9pt}
% \section{Introduction}
% \label{sec:intro}
% %\vspace{-5pt}
% Deep learning models are a quintessential example of black box methods where it is very hard to see why the model generates the output it does. Over recent years, there has been a rise in the need for explainable deep learning models that have led to several efforts~\cite{Guan2019TowardsAD,Liu2018TowardsEN,Gilpin2018ExplainingEA,Chen2018ExplainingNN,Yosinski2015UnderstandingNN,Sharp2017TellMW,Ghosh2019GeneratingN,Hu2018ExplainableNC}; however, the need to generate a human-understandable justification for the decisions of a neural network model has remained. In this work, we propose a new task and methodology for automatically generating answer and rationale for a visual question, thus going beyond traditional Visual Question Answering~\cite{Antol2015VQAVQ}.
% 
% Visual Question Answering (VQA)~\cite{Thomason2018ShiftingTB,Lu2019ViLBERTPT,Storks2019CommonsenseRF} is a vision-language task that has seen a lot of attention in recent years. There are an increasing number of models devoted to obtaining the best possible performance on benchmark VQA datasets, which intend to measure visual understanding based on visual questions. Also, more recently, the Visual Commonsense Reasoning (VCR) task~\cite{Zellers2018FromRT,Lu2019ViLBERTPT,Dua2019DROPAR,Zheng2019ReasoningVD,Talmor2018CommonsenseQAAQ,Lin2019KagNetKG} has been proposed, which requires a greater level of visual understanding and an ability to reason about the world. However, both these tasks are posed as multiple-choice questions, which in effect, reduces them to classification problems, i.e., models which solve these tasks simply need to pick an answer in the case of VQA, or an answer and a rationale for VCR. Such models may be prone to memorization or lack high-level visual reasoning itself. Efforts towards making such models less opaque have been undertaken, for example, by VQA-E~\cite{Li2018VQAEEE} via making the model generate an explanation for its answer choice. However, the answers in VQA are often binary, and the problem persists with regards to questions of the type 'why' and 'how', since the generated explanations need to be at an object level. To go beyond the contemporary efforts, we propose, for the first time to the best of our knowledge, a task that requires the automatic generation of both answer and an accompanying rationale that seeks to explain the said answer for a given visual query. We term this task \pnamefull(\pname). We also propose an end-to-end methodology to address this task.
% 
% Our model to address this task consists of four sequentially arranged recurrent networks. The model can be seen as having two parts: a generation module (GM), which comprises of the first two sequential recurrent networks, and a refinement module (RM), which comprises of the final two sequential recurrent networks. The GM first generates an answer, using which it generates a rationale that explains the answer. The RM generates a \textit{refined} answer based on the rationale generated by GM. The refined answer is further used to generate a refined rationale. Our model is motivated by the way humans think about answers to questions, wherein the answer and rationale are often mutually dependent on each other. We seek to model this cyclic dependency by first generating the answer-rationale pair, and then using them as priors to regenerate a refined answer and rationale. We train our model on the VCR dataset, which contains open-ended visual questions along with answers and rationales. Considering this is a generative task, we evaluate our methodology by comparing our generated
% answer/rationale with the ground truth answer/rationale on correctness and goodness of the generated content, as well as by human Turing Tests. Considering the difficulty of this task, we observe promising qualitative and quantitative results, as presented later in this paper.
% 
% Our main contributions in this work are three-fold: (i) Firstly, we propose a new task \pname that aims to provide a new direction to interpretable models that can perform visual reasoning and provide human-understandable rationale; (ii) Secondly, we propose an end-to-end methodology for \pname, obtain promising results, and perform ablation studies on our methodology to study its effectiveness on \pname; and (iii) We discuss how to evaluate such models, and provide performance metrics for this task. We believe that this work could lead to further efforts on human-understandable answer and rationale generation in vision tasks in the near future.

==> CVPR/sections/related_copy.tex <==
%\vspace{-18pt}
\section{Related Work}
\label{sec:related}
%\vspace{-6pt}
In this section, we review earlier efforts from multiple perspectives that may be related to this work: Visual Question Answering, Visual Commonsense Reasoning and Image Captioning in general.
% 
%\vspace{-12pt}
\noindent \paragraph{\textbf{Visual Question Answering (VQA):}}
VQA~\cite{Antol2015VQAVQ,Goyal2016MakingTV,Jabri2016RevisitingVQ,Selvaraju2020SQuINTingAV} refers to the task of answering questions related to an image. VQA and its variants have been the subject of much research work recently. A lot of recent work has focused on varieties of attention-based models, which aim to 'look' at the relevant regions of the image in order to answer the question ~\cite{DBLP:journals/corr/AndersonHBTJGZ17,Lu2016HierarchicalQC,Yu2017MultilevelAN,Xu2015AskAA,Yi2018NeuralSymbolicVD,Xu2015AskAA,Shih2015WhereTL,DBLP:journals/corr/ChenWCGXN15,Yang2015StackedAN}. Other recent work has focused on better multimodal fusion methods~\cite{Kim2018BilinearAN,DBLP:journals/corr/KimOKHZ16,Fukui2016MultimodalCB,Yu2017MultimodalFB}, the
incorporation of relations~\cite{NorcliffeBrown2018LearningCG,Li2019RelationAwareGA,Santoro2017ASN}, the use of multi-step reasoning~\cite{Cadne2019MURELMR, Gan2019MultistepRV, Hudson2018CompositionalAN},  and neural module
networks for compositional reasoning~\cite{Johnson2017InferringAE,Chen_2021_WACV,Hu2017LearningTR}. Visual Dialog~\cite{Das2018VisualD,Zheng2019ReasoningVD} extends VQA but requires an agent to hold a meaningful conversation with humans in natural language based on visual questions.
%Despite good performance, the most such models can present in way of explainability are attention maps. 

The efforts closest to ours are those that provide justifications along with answers~\cite{Li2018VQAEEE,Hendricks2016GeneratingVE,Li2018TellandAnswerTE,Park2018MultimodalEJ,Wu2019GeneratingQR,Park2018MultimodalEJ,Mooney2017EnsemblingVE}, each of which however also answers a question as a classification task (and not in a generative manner) as described below. ~\cite{Li2018VQAEEE} create the VQA-E dataset that has an explanation along with the answer to the question. \cite{Wu2019GeneratingQR} provide relevant captions to aid in solving VQA, which can be thought of as weak justifications. More recent efforts~\cite{Park2018MultimodalEJ,Patro2020RobustEF} attempt to provide visual and textual explanations to justify the predicted answers. Datasets have also been proposed for VQA in the recent past to test visual understanding \cite{Zhu2015Visual7WGQ,Goyal2016MakingTV,Johnson2016CLEVRAD}; for e.g., the Visual7W dataset~\cite{Zhu2015Visual7WGQ} contains a richer class of questions about an image with textual and visual answers. However, all these aforementioned efforts continue to focus on answering a question as a classification task (often in one word, such as Yes/No), followed by simple explanations. We however, in this work, focus on \textit{generating} multi-word answers with a corresponding multi-word rationale, which has not been done before. 
% However, the answers in these are open-ended(generally yes/no, numerical, single-word answers), and the problem persists since all the questions cannot be answered with one word and existing work (VQA-E and Multi-modal explanation) fails to provide  multi-word answers.
%\textbf{BERT: }Bidirectional Encoder Representations from Transformers~\cite{Devlin2019BERTPO} state-of-the-art results in a wide variety of NLP tasks, including Question Answering. BERT can be used to obtain sentence embeddings that are contextual. The vector representation of a token depends on the other words in the sequence, in both directions. We have used the same to obtain sentence level contextual embedding for give question and image caption. Contextual embeddings capture greater linguistic information than token level embeddings.
% 
%\vspace{-12pt}
\noindent \paragraph{\textbf{Visual Commonsense Reasoning (VCR):}}
VCR \cite{Zellers2018FromRT} is a recently introduced vision-language dataset which involves choosing a correct answer (among four provided options) for a given question about the image, and then choosing a rationale (among four provided options) that justifies the answer. The task associated with the dataset aims to test for visual commonsense understanding and provides images, questions and answers of a higher complexity than other datasets such as CLEVR \cite{Johnson2016CLEVRAD}. The dataset has attracted a few methods over the last year~\cite{Zellers2018FromRT,Lu2019ViLBERTPT,Dua2019DROPAR,Zheng2019ReasoningVD,Talmor2018CommonsenseQAAQ,Lin2019KagNetKG,Lin2019TABVCRTA,Wu2019ConnectiveCN,Ayyubi2019EnforcingRI,Brad2019SceneGC,Yu2019HeterogeneousGL,Wu2019ConnectiveCN}, each of which however follow the dataset's task and treat this as a classification problem. None of these efforts attempt to answer and reason using generated sentences.% 
%\vspace{-12pt}
\noindent \paragraph{\textbf{Image Captioning and Visual Dialog:}} One could also consider the task of image captioning~\cite{Xu2015ShowAA,You2016ImageCW,Lu2016KnowingWT,DBLP:journals/corr/AndersonHBTJGZ17,Rennie2016SelfCriticalST}, where natural language captions are generated to describe an image, as being close to our objective. However, image captioning is more a global description of an image than question-answering problems that may be tasked with answering a question about understanding of a local region in the image.

%Such a task has an additional layer of complexity to it, since first and foremost, the generated text has to be structurally correct. Further, an image captioning model needs to generate grammatically correct captions, even if its visual understanding is lacking. %Most captioning architectures are attention based encoder-decoder architectures ~\cite{Xu2015ShowAA,You2016ImageCW,Lu2016KnowingWT,Anderson2017BottomUpAT, Rennie2016SelfCriticalST}.
  %\cite{Anderson2017BottomUpAT} introduce object-level image features as bottom-up-attention. ~\cite{Lu2016KnowingWT} proposes soft spatial attention, which is the top-down attention of choice in ~\cite{Anderson2017BottomUpAT}. 
% 

In contrast to all the aforementioned efforts, our work, \pname, focuses on automatic complete \textit{generation} of the answer, and of a rationale, given a visual query. This is a challenging task, since the generated answers must be correct (with respect to the question asked), be complete, be natural, and also be justified with a well-formed rationale. We now describe the task, and our methodology for addressing this task.
